WONDERBREAD: A Benchmark for Evaluating Multimodal Foundation Models on Business Process Management Tasks

Existing ML benchmarks lack the depth and diversity of annotations needed for evaluating models on business process management (BPM) tasks. BPM is the practice of documenting, measuring, improving, and automating enterprise workflows. However, research has focused almost exclusively on one task - full end-to-end automation using agents based on multimodal foundation models (FMs) like GPT-4. This focus on automation ignores the reality of how most BPM tools are applied today - simply documenting the relevant workflow takes 60% of the time of the typical process optimization project. To address this gap we present WONDERBREAD, the first benchmark for evaluating multimodal FMs on BPM tasks beyond automation. Our contributions are: (1) a dataset containing 2928 documented workflow demonstrations; (2) 6 novel BPM tasks sourced from real-world applications ranging from workflow documentation to knowledge transfer to process improvement; and (3) an automated evaluation harness. Our benchmark shows that while state-of-the-art FMs can automatically generate documentation (e.g. recalling 88% of the steps taken in a video demonstration of a workflow), they struggle to re-apply that knowledge towards finer-grained validation of workflow completion (F1 < 0.3). We hope WONDERBREAD encourages the development of more "human-centered" AI tooling for enterprise applications and furthers the exploration of multimodal FMs for the broader universe of BPM tasks. We publish our dataset and experiments here: https://github.com/HazyResearch/wonderbread

==> Intro_PM.tex <==
\section{Introduction}

Artificial intelligence is projected to increase overall global productivity by up to 3.4\% compounded annually through 2040 \cite{chui2023economic}. Large Multimodal Models (LMMs) such as GPT4-V have shown early promise in delivering such enterprise value \cite{hypecyclegartner} as they possess robust world knowledge reasoning, and planning skills \cite{gpt4, zhang2023visionlanguage, yao2022react, tu2023generalist, cogagent}.

% What is the problem?

% Why is it interesting and important?
% Why is it hard? (E.g., why do naive approaches fail?)
% Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)
% What are the key components of my approach and results? Also include any specific limitations.

Process mining is one such valuable application  \cite{dumas2023ai}. Process mining is essentially an organizational "X-Ray" \cite{reinkemeyer2020process} which enables large enterprises to identify, understand, and improve their workflows \cite{van2014process, reinkemeyer2020process, augusto2018automated}. Effective process mining can have a multiplier effect on productivity, and the business process management market is projected to reach \$65 billion by 2032 \cite{fahland2024well}.

Despite several case studies showing promise, the application of LMMs to process mining remains underexplored \cite{fahland2024well, berti2023leveraging}. Instead, current tools typically focus on converting textual event logs (i.e. clickstreams) into graphical visualizations of a workflow \cite{augusto2018automated}. These tools struggle to understand higher-level semantics and workflow abstractions, with a common failure mode being "spaghetti-like” outputs which are too low-level to offer insights \cite{agostinelli2020towards, leno2021robotic, van2021event, agostinelli2020towards, augusto2018automated, fahland2024well}. In practice, these tools must usually be paired with domain experts and trained process modellers to be used successfully, which can take significant time and effort \cite{grohs2023large}; simply defining the correct process model is estimated to take up to 60\% of the time of a process management project \cite{friedrich2011process}

Given their world knowledge and multimodal reasoning abilities, we ask: \textbf{To what extent can LMMs mimic the way humans understand and explain business processes via visual observation and natural language?}

We refer to this as \textbf{“observational process mining”}, with the goal of achieving \textbf{“workflow understanding”} in the same vein as other machine learning subfields focused on “natural language understanding” or “image understanding.” 

In contrast to traditional process mining, we propose that observational process mining uses LMMs to ingest a wide range of multimodal process captures that exist in enterprise environments (e.g. videos, clickstreams, application metadata, written documents, etc.) \cite{vidgof2023large, rizk2023case} while generating semantically meaningful workflow documentation. In doing so, observational process mining can bridge the “semantic gap” that currently exists between process mining tools and human workflow understanding \cite{fahland2024well}.

A key roadblock in measuring an LMM's ability to understand workflows is the lack of existing benchmarks and datasets \cite{vidgof2023large}. While a number of datasets for process mining exist \cite{augusto2018automated}, they have several key limitations. 
\begin{enumerate}
    \item \textbf{Single Modality:} Most benchmarks almost exclusively focus on low-level event logs (e.g. no screen recordings, written documentation, etc.).
    \item \textbf{Semantic Gap:} Methods are typically evaluated on their ability to generate low-level representations of workflows (e.g. Petri nets, BPMs, etc.), which can be difficult for humans to parse and do not represent true “understanding” of a workflow.
    \item \textbf{Limited Application:} Current benchmarks and evaluation metrics neglect one of the primary purposes of process mining -- automation.
\end{enumerate}

An ideal benchmark for observational process mining would contain multimodal data, capture semantic task-knowledge, and provide an automated evaluation harness coupled with a downstream automation use case. 

As a first step towards this vision, we introduce \dataset, a dataset and benchmark aimed at bridging the semantic gap between human and machine process modeling by focusing on the three core value propositions of process modeling: (1) process identification, (2) process understanding, and (3) process monitoring. As we advocate for a tighter coupling between model outputs and human abstractions, \dataset evaluates LMMs on their ability to generate interpretable written documentation such as standard operating procedures (“SOPs”) rather than traditional process mining outputs such as Petri nets or BPMNs.

\dataset is a collection of \todo{XX} human task demonstrations (full screen recordings, action traces, and manually written documentation) for \todo{XX} web navigation tasks sourced from the WebArena benchmark \cite{zhou2023webarena}. The contributions of \dataset are as follows:

\begin{enumerate}
    \item \textbf{Dataset:} A dataset which contains \todo{XX} human task demonstrations across \todo{XX} web navigation tasks. We source demonstrations from \todo{XX} independent annotators for each task, thus providing a diversity of traces. The dataset is multimodal, as each demonstration contains a full screen recording and event log, as well as a manually written step-by-step guide (“SOP”) reflecting the human annotator’s understanding of the workflow. 
    \item \textbf{Benchmark:} A benchmark targeting the three components of observational process mining: task identification, understanding and monitoring. We define a total of \todo{XX} tasks.
    \item \textbf{Evaluation:} An automated evaluation harness for model-generated SOPs, as well as an end-to-end evaluation framework which uses an autonomous agent to solve the documented workflow. We show alignment with human evaluators, and provide baseline results with GPT4-V that show \todo{XXX} performance.
\end{enumerate}

The rest of the paper is structured as follows. \todo{TODO}

To summarize, the contributions of \dataset{} are as follows: a dataset for evaluating observational process mining, a comprehensive benchmark and automated evaluation harness, and initial results with the current state-of-the-art LMM (GPT-4V). 


Defining what it means to "understand" a workflow is challenging, as workflows often contain many levels of abstraction and typically have a wide space of semantically equivalent formulations. For example, the step \textit{"Delete the record for patient X"} can either be broken down into many individual steps (e.g. \textit{"Click the patient list -> Scroll down until X is visible -> Click the dropdown menu -> Select the 'Delete' option"})  or aggregated upwards (e.g. as part of the broader action \textit{"Clear the entire patient list"}). Additionally, there are often many possible ways to successfully accomplish a given objective, which means that assessing the "correctness" of a workflow depends not only on the individual steps taken, but the larger context in which it is executed.




Despite growing interest in these capabilities \cite{fahland2024well, rizk2023case, dumas2023ai, vidgof2023large, berti2023leveraging, grohs2023large, muthusamy2023towards}, existing benchmarks and datasets have several key limitations:

\begin{enumerate}
    \item \textbf{Single Modality:} Datasets contain event logs (e.g. clickstreams) of a process without accompanying screen recordings or written documentation. This neglects the key strengths of an LMM.
    \item \textbf{Semantic Gap:} Methods are assessed on their ability to generate low-level representations of a workflow (e.g. Petri nets, BPMs, etc.) rather than their ability to form higher-level abstractions and generate human-interpretable outputs. In other words, they lose the forest for the trees.
    \item \textbf{Limited Manual Evaluation:} Benchmarks rely heavily on human evaluation of discrete subcomponents of a workflow and do not measure the most exciting manifestation of workflow understanding -- namely, going from raw demonstrations to full end-to-end task automation.
\end{enumerate}




\begin{enumerate}
    \item \textbf{Process Mining Benchmarks:} These are single modality, semantic gap, manual evaluation. However, they do a good job of assessing canonical "workflow understanding".
    \item \textbf{Web Navigation Benchmarks:} These are interactive, multimodal, and support automated evaluations. However, they do not measure the various aspects of workflow understanding (instead focusing entirely on end-to-end task completion) and do not incorporate domain knowledge or human reference demonstrations.
\end{enumerate}




\begin{enumerate}
    \item \textbf{Process Mining Benchmarks:} These are single modality, semantic gap, manual evaluation. However, they do a good job of assessing canonical "workflow understanding".
    \item \textbf{Web Navigation Benchmarks:} These are interactive, multimodal, and support automated evaluations. However, they do not measure the various aspects of workflow understanding (instead focusing entirely on end-to-end task completion) and do not incorporate domain knowledge or human reference demonstrations.
\end{enumerate}





\begin{enumerate}
    \item \textbf{Task Identification} (aka "segmentation" / "session mining" / "intention mining") -- Segmenting a long trace of actions (which can potentially involve many separate tasks) into a set of discrete tasks \cite{agostinelli2020towards, leno2021robotic, ghasemi2020event, vidgof2023large}.
    \item \textbf{Task Understanding} (aka "(sub)routine identification" / "simplification" / "noise filtering") -- Identifying the semantically meaningful clusters of actions required to execute a task. Key challenges include the high level of noise in action traces, as well as the fact that many routines are performed in somewhat arbitrary orderings (e.g. filling out a form) which makes pattern-matching difficult \cite{leno2021robotic, vidgof2023large}.
    \item \textbf{Task Monitoring} (aka "enhancement") -- Discovering inefficiencies in the workflow, proposing ways to improve it, and automatically detecting errors \cite{ghasemi2020event, vidgof2023large, leno2021robotic}. A key challenge is there are often many valid ways to perform the same workflow, and the optimal set of steps can be input dependent. \cite{leno2021robotic}.
\end{enumerate}














% Existing benchmarks have tasks, but don’t show you what’s happening under the covers (i.e. human understanding)
human demonstrations enable for:
Documenting task processes -- i.e. what is happening
Transferring expert knowledge -- i.e. how does someone new (AI or human) learn how to do an existing task
Improving processes -- i.e. given an existing workflow, how to make it better
document, transfer, improve 
Here’s why this intermediate representation matters [HBS stuff] (try to parallel this with the three bullets)
Documenting -- regulatory requirements, auditing, ensuring consistency
Transferring -- onboard new hires, upskill existing workers
Improving -- increase productivity
Here’s how our dataset answers this question



% Why is it hard? (E.g., why do naive approaches fail?)
% Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)
In the same vein as "natural language understanding", we coin the phrase \textbf{``workflow understanding''} to refer to the ability of LMMs to identify, analyze, and improve business processes. 

Despite growing interest in these capabilities \cite{fahland2024well, rizk2023case, dumas2023ai, vidgof2023large, berti2023leveraging, grohs2023large, muthusamy2023towards}, existing benchmarks and datasets for LMMs \cite{mmnavigator_gpt4v_in_wonderland, zhou2023webarena, webvoyager, wu2024copilot, zhang2024ufo} do not model the key attributes of enterprise settings:

\begin{enumerate}
    \item \textbf{Domain Expertise:} Enterprise workflows typically require training, and operate at several levels of abstraction \cite{brynjolfsson2023generative, autor2014polanyi}. However, existing datasets of human task demonstrations lack such supervision -- i.e. they do not contain labels of what the human annotators were thinking as they demonstrated workflows, making it impossible to train or evaluate models on them.
    \item \textbf{Collective Knowledge:} Enterprise workflows are completed by teams of individuals with differing approaches and efficiencies \cite{brynjolfsson2023generative}. Existing datasets don't release multiple demonstrations from different annotators for the same task, which prevents them from realistically modeling the diversity of processes within enterprise settings. 
    \item \textbf{Process Understanding:} Beyond end-to-end automation, an LMM's workflow understanding abilities could provide value to enterprises via automated process documentation, onboarding new hires, cross-team knowledge transfer, creating training docs, process mining, etc. \cite{leno2021robotic}. Existing benchmarks, however, tend to exclusively focus on end-to-end task automation and neglect the various sub-components of workflow understanding.
\end{enumerate}

Our work aims to address this gap by providing a benchmark to help answer the question: \textbf{To what extent can LMMs mimic the way humans understand and explain business processes via visual inspection and natural language?}

As a first step towards this vision, we introduce \dataset{} -- a collection of \todo{3,000} human task demonstrations (full screen recordings, action traces, and manually written step-by-step guides) for \todo{500} web navigation tasks sourced from the WebArena benchmark \cite{zhou2023webarena}. \dataset{} helps bridge the gap between enterprise settings and prior work on using LMMs for task automation through the following contributions:

\begin{enumerate}
    \item \textbf{Domain Expertise:} \dataset{} provides \todo{3000} human task demonstrations across \todo{500} web navigation tasks and \todo{4} websites. Each demonstration contains a full screen recording and a step-by-step guide ("SOP") written by the human annotator. The SOPs enable us to measure the gap between a human's and model's abstractions for the same workflow. They also enable us to test incorporation of domain knowledge into a model. 

    \item \textbf{Collective Knowledge:} \dataset{} provides demonstrations from \todo{4} independent human annotators for each task, and has annotators rank the demonstrations on their relative quality. We do rigorous QA to ensure data is high quality and reflective of ``expert-level'' task executions. This better reflects the diversity of real-world enterprises which have many individual contributors.

    \item \textbf{Process Understanding:} \dataset{} provides an automated evaluation harness to measure the three distinct components of workflow understanding -- identification, understanding, and monitoring -- across which we provide \todo{6} distinct tasks. We show alignment of our automated evaluations with human evaluators, and provide baseline results with GPT4-V that show \todo{XXX} performance.
\end{enumerate}




% It evaluates three core components of workflow understanding: (1) identification, (2) analysis, and (3) monitoring. 

    % We solve by providing human-written SOPs corresponding to each video demonstration, which enables measuring the gap between how humans and models create abstractions to understand the same workflow. The SOPs also allow for testing how to incorporate domain knowledge into the model. Finally, we do a rigorous QA check to ensure demos are high quality and SOPs reflect "domain expertise"

    % We solve by collecting multiple human demonstrations and SOPs for each task, and having human annotators provided an ordered ranking for each task's demonstrations.

    %We solve by constructing a robust benchmark with 6 tasks, measuring the ability of models to identity, analyze and monitor tasks. 


% As we advocate for a tighter coupling between model and human workflow understanding, \dataset{} evaluates LMMs on their ability to generate interpretable written documentation such as standard operating procedures (“SOPs”) rather than traditional process mining outputs such as Petri nets or BPMN models.

% \dataset{} is a collection of \todo{3,000} total human task demonstrations (full screen recordings, action traces, and manually written SOPs) for \todo{500} web navigation tasks sourced from the WebArena benchmark \cite{zhou2023webarena}. The contributions of \dataset are as follows:

% \begin{enumerate}
%     \item \textbf{Dataset:} A dataset which contains \todo{3000} human task demonstrations across \todo{500} web navigation tasks and \todo{4} websites. Each task has an average of \todo{10} steps. We source demonstrations from \todo{4} independent human annotators for each task, thus providing a diversity of traces. Each demonstration contains a full screen recording, event log of all clicks/keystrokes/scrolls, and a manually written SOP reflecting the human annotator’s understanding of the workflow. The average screen recording is \todo{30} seconds, and the average event log contains \todo{12} actions.
%     \item \textbf{Benchmark:} A benchmark targeting three components of workflow understanding: identification, understanding and monitoring. We define a total of \todo{6} distinct tasks.
%     \item \textbf{Evaluation:} An automated evaluation harness for model-generated SOPs, as well as an end-to-end evaluation framework which uses an autonomous agent to execute the documented workflow. We show alignment with human evaluators, and provide baseline results with GPT4-V that show \todo{XXX} performance.
% \end{enumerate}

The rest of the paper is structured as follows. \todo{TODO}

To summarize, the contributions of \dataset{} are as follows: (1) a dataset for evaluating workflow understanding, (2) a comprehensive benchmark of the three subcomponents of workflow understanding (3) an automated evaluation harness, and (4) initial results with state-of-the-art LMMs such as GPT4-V and Gemini Pro.




% What are the key components of my approach and results? Also include any specific limitations.

% Workflow understanding requires a unique blend of common sense, causal reasoning, multimodal understanding, and world knowledge about how human organizations function. Despite growing interest in using LMMs for tasks such as process mining and task automation \cite{fahland2024well, rizk2023case, dumas2023ai, vidgof2023large, muthusamy2023towards}, such capabilities remains underexplored as they are difficult to define and quantitatively measure \cite{vidgof2023large}.




% We have models that have special skills. They have already shown the ability to automate some tasks. We'd like to know whether they can understand these processes. 


% Ppl are focused on the wrong thing -- individual use cases instead of enterprise scenarios.

% LMMs are quickly becoming integral actors in the enterprise.~\citep{} showing the promise of automating the enterprise. 

% \todot{The dream is automating the enterprise. Understand what's happening, automate it, and improve it.}

% Artificial intelligence is projected to increase overall global productivity by up to 3.4\% compounded annually through 2040 \cite{chui2023economic}.

% Improving how these organizations function could unlock significant value -- the business process management market is
% projected to reach \$65 billion by 2032 \cite{fahland2024well}. 





% Why is it hard? (E.g., why do naive approaches fail?)
% Defining what it means to "understand" a workflow is challenging, as workflows often contain many levels of abstraction (e.g. \textit{Delete the record for patient X} can be broken down into \textit{Click the patient list -> Scroll down until X is visible -> Click the dropdown menu -> Select the 'Delete' option}) and typically have a wide space of semantically equivalent formulations (e.g. \textit{Cmd+C} has the same effect as right clicking and clicking \textit{Copy}) \cite{augusto2018automated, leno2021robotic, van2021event}.

% Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)

% Individual v. team

 % LMMs could ingest a broad range of multimodal process captures (e.g. videos, clickstreams, application metadata, written documents, etc.) \cite{vidgof2023large, rizk2023case} generate interpretable analyses and documentation, and eventually fully automate tasks, thereby bridging the "semantic gap" that currently exists between traditional workflow understanding tools (e.g. process mining) and human workflow understanding \cite{fahland2024well}. 


% Despite several case studies showing promise, the application of LMMs to process mining remains underexplored \cite{fahland2024well, berti2023leveraging}. Instead, current tools typically focus on converting textual event logs (i.e. clickstreams) into graphical visualizations of a workflow \cite{augusto2018automated}. These tools struggle to understand higher-level semantics and workflow abstractions, with a common failure mode being "spaghetti-like” outputs which are too low-level to offer insights \cite{agostinelli2020towards, leno2021robotic, van2021event, agostinelli2020towards, augusto2018automated, fahland2024well}. In practice, these tools must usually be paired with domain experts and trained process modellers to be used successfully, which can take significant time and effort \cite{grohs2023large}; simply defining the correct process model is estimated to take up to 60\% of the time of a process management project \cite{friedrich2011process}



    % \item \textbf{Documentation:} For each of the 3,023 demonstrations in \dataset{}, the human annotator writes a step-by-step guide ("SOP") outlining their thoughts as they completed the workflow. This allows us to track how a human thinks through each step and compare against model-generated documentation.
    % \item \textbf{Knowledge Transfer:} We develop Each task contains an average of 5 separate human demonstrations. For 179 of these tasks, an annotator manually ranks each human demonstration from highest to lowest quality. Using these demonstrations, we measure the models ability to do XX demonstrating 
    
    %We do rigorous QA to ensure data is high quality and reflective of ``expert-level'' task executions. This better reflects the diversity of real-world enterprises which have many individual contributors. (mulitple sop --> sop, sop, generationg, e2e completion rate given sop)

    % \item \textbf{Process Improvement:} Each task contains an average of 5 separate human demonstrations. For 179 of these tasks, an annotator manually ranks each human demonstration from highest to lowest quality. We also create a question answering


% It evaluates three core components of workflow understanding: (1) identification, (2) analysis, and (3) monitoring. 

    % We solve by providing human-written SOPs corresponding to each video demonstration, which enables measuring the gap between how humans and models create abstractions to understand the same workflow. The SOPs also allow for testing how to incorporate domain knowledge into the model. Finally, we do a rigorous QA check to ensure demos are high quality and SOPs reflect "domain expertise"

    % We solve by collecting multiple human demonstrations and SOPs for each task, and having human annotators provided an ordered ranking for each task's demonstrations.

    %We solve by constructing a robust benchmark with 6 tasks, measuring the ability of models to identity, analyze and monitor tasks. 

% \dataset{} provides an automated evaluation harness to measure the three distinct components of workflow understanding -- identification, understanding, and monitoring -- across which we provide \todo{6} distinct tasks. We show alignment of our automated evaluations with human evaluators, and provide baseline results with GPT4-V that show \todo{XXX} performance.


% As we advocate for a tighter coupling between model and human workflow understanding, \dataset{} evaluates LMMs on their ability to generate interpretable written documentation such as standard operating procedures (“SOPs”) rather than traditional process mining outputs such as Petri nets or BPMN models.

% \dataset{} is a collection of \todo{3,000} total human task demonstrations (full screen recordings, action traces, and manually written SOPs) for \todo{500} web navigation tasks sourced from the WebArena benchmark \cite{zhou2023webarena}. The contributions of \dataset are as follows:

% \begin{enumerate}
%     \item \textbf{Dataset:} A dataset which contains \todo{3000} human task demonstrations across \todo{500} web navigation tasks and \todo{4} websites. Each task has an average of \todo{10} steps. We source demonstrations from \todo{4} independent human annotators for each task, thus providing a diversity of traces. Each demonstration contains a full screen recording, event log of all clicks/keystrokes/scrolls, and a manually written SOP reflecting the human annotator’s understanding of the workflow. The average screen recording is \todo{30} seconds, and the average event log contains \todo{12} actions.
%     \item \textbf{Benchmark:} A benchmark targeting three components of workflow understanding: identification, understanding and monitoring. We define a total of \todo{6} distinct tasks.
%     \item \textbf{Evaluation:} An automated evaluation harness for model-generated SOPs, as well as an end-to-end evaluation framework which uses an autonomous agent to execute the documented workflow. We show alignment with human evaluators, and provide baseline results with GPT4-V that show \todo{XXX} performance.
% \end{enumerate}



% What are the key components of my approach and results? Also include any specific limitations.

% Workflow understanding requires a unique blend of common sense, causal reasoning, multimodal understanding, and world knowledge about how human organizations function. Despite growing interest in using LMMs for tasks such as process mining and task automation \cite{fahland2024well, rizk2023case, dumas2023ai, vidgof2023large, muthusamy2023towards}, such capabilities remains underexplored as they are difficult to define and quantitatively measure \cite{vidgof2023large}.




% We have models that have special skills. They have already shown the ability to automate some tasks. We'd like to know whether they can understand these processes. 


% Ppl are focused on the wrong thing -- individual use cases instead of enterprise scenarios.

% LMMs are quickly becoming integral actors in the enterprise.~\citep{} showing the promise of automating the enterprise. 

% \todot{The dream is automating the enterprise. Understand what's happening, automate it, and improve it.}

% Artificial intelligence is projected to increase overall global productivity by up to 3.4\% compounded annually through 2040 \cite{chui2023economic}.

% Improving how these organizations function could unlock significant value -- the business process management market is
% projected to reach \$65 billion by 2032 \cite{fahland2024well}. 





% Why is it hard? (E.g., why do naive approaches fail?)
% Defining what it means to "understand" a workflow is challenging, as workflows often contain many levels of abstraction (e.g. \textit{Delete the record for patient X} can be broken down into \textit{Click the patient list -> Scroll down until X is visible -> Click the dropdown menu -> Select the 'Delete' option}) and typically have a wide space of semantically equivalent formulations (e.g. \textit{Cmd+C} has the same effect as right clicking and clicking \textit{Copy}) \cite{augusto2018automated, leno2021robotic, van2021event}.

% Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)

% Individual v. team

 % LMMs could ingest a broad range of multimodal process captures (e.g. videos, clickstreams, application metadata, written documents, etc.) \cite{vidgof2023large, rizk2023case} generate interpretable analyses and documentation, and eventually fully automate tasks, thereby bridging the "semantic gap" that currently exists between traditional workflow understanding tools (e.g. process mining) and human workflow understanding \cite{fahland2024well}. 


% Despite several case studies showing promise, the application of LMMs to process mining remains underexplored \cite{fahland2024well, berti2023leveraging}. Instead, current tools typically focus on converting textual event logs (i.e. clickstreams) into graphical visualizations of a workflow \cite{augusto2018automated}. These tools struggle to understand higher-level semantics and workflow abstractions, with a common failure mode being "spaghetti-like” outputs which are too low-level to offer insights \cite{agostinelli2020towards, leno2021robotic, van2021event, agostinelli2020towards, augusto2018automated, fahland2024well}. In practice, these tools must usually be paired with domain experts and trained process modellers to be used successfully, which can take significant time and effort \cite{grohs2023large}; simply defining the correct process model is estimated to take up to 60\% of the time of a process management project \cite{friedrich2011process}

